A Class of Parallel Doubly Stochastic Algorithms for Large-Scale Learning

We consider learning problems over training sets in which both, the number of training examples and the dimension of the feature vectors, are large. To solve these problems we propose the random parallel stochastic algorithm (RAPSA). We call the algorithm random parallel because it utilizes multiple parallel processors to operate on a randomly chosen subset of blocks of the feature vector. We call the algorithm stochastic because processors choose training subsets uniformly at random. Algorithms that are parallel in either of these dimensions exist, but RAPSA is the first attempt at a methodology that is parallel in both the selection of blocks and the selection of elements of the training set. In RAPSA, processors utilize the randomly chosen functions to compute the stochastic gradient component associated with a randomly chosen block. The technical contribution of this paper is to show that this minimally coordinated algorithm converges to the optimal classifier when the training objective is convex. Moreover, we present an accelerated version of RAPSA (ARAPSA) that incorporates the objective function curvature information by premultiplying the descent direction by a Hessian approximation matrix. We further extend the results for asynchronous settings and show that if the processors perform their updates without any coordination the algorithms are still convergent to the optimal argument. RAPSA and its extensions are then numerically evaluated on a linear estimation problem and a binary image classification task using the MNIST handwritten digit dataset.

==> Convergence2.tex <==
%!TEX root = root.tex
\section{Convergence analysis}\label{sec_convergence}





Our goal here is to show that as time progresses the sequence of iterates $\bbx^t$ approaches the optimal argument $\bbx^*$. To do so, in addition to the conditions on the weight matrices $\bbW$ and $\tbW$ in Assumption \ref{ass_wight_matrix_conditions}, we assume the instantaneous local functions $f_{n,i}$ have specific properties that we state next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    R   E   M    A    R    K      %%%%% %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{remark}
%Note that given the weight matrix $\bbW$ that satisfies conditions in Assumptions \ref{ass_wight_matrix_conditions}\eqref{decentralized}-\ref{ass_wight_matrix_conditions}\eqref{spectral1}, the trivial choice for $\tbW$ that satisfies all the condition in Assumptions \ref{ass_wight_matrix_conditions}\eqref{decentralized}-\ref{ass_wight_matrix_conditions}\eqref{spectral2} is 
%%%%
%\begin{equation}\label{special_case_of_tbW}
%\tbW=\frac{\bbI+\bbW}{2}.
%\end{equation}
%%%
%Therefore, different weight (mixing) rules can be applied for designing the weight matrices $\bbW$ e.g. Metropolis, Laplacian-based, and weight matrix $\tbW$ can be generated as in \eqref{special_case_of_tbW}.
%\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    M  A   I  N         M   A    T   T   E   R  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   S   S   U   M   P   T   I   O   N    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{assumption}\label{ass_intantaneous_hessian_bounds}\normalfont  The instantaneous local functions $f_{n,i}(\bbx_n)$ are differentiable and strongly convex with parameter $\mu$.
\end{assumption}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   S   S   U   M   P   T   I   O   N    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{assumption}\normalfont\label{ass_bounded_stochastic_gradient_norm} 
The gradient of instantaneous local functions $\nabla f_{n,i}$ are Lipschitz continuous with parameter $L$. I.e., for all $n\in\{1,\dots,N\}$ and $i\in\{1,\dots,q_n\}$ we can write
\begin{equation}
\left\|\nabla f_{n,i}(\bba)-\nabla f_{n,i}(\bbb)\right\| \leq L\ \| \bba-\bbb \|\quad\!  \bba,\bbb \in \reals^p.
\end{equation}
\end{assumption}

The condition imposed by Assumption \ref{ass_intantaneous_hessian_bounds} implies that the local functions $f_{n}(\bbx_{n})$ and the global cost function $f(\bbx)=\sum_{n=1}^N f_{n}(\bbx_{n})$ are also strongly convex with parameter $\mu$. Likewise, Lipschitz continuity of the local instantaneous gradients considered in Assumption \ref{ass_bounded_stochastic_gradient_norm} enforces Lipschitz continuity of gradients of the local functions $\nabla f_n(\bbx_n)$ and the aggregate function $\nabla f(\bbx)$ -- see, e.g., (Lemma 1 of \cite{mokhtari2015network}).

\subsection{Preliminaries}

In this section we study some basic properties of the sequences of primal and dual variables generated by the DSA algorithm. In the following lemma, we study the relation of iterates $\bbx^t$ and $\bbv^t$ with the optimal primal  $\bbx^*$ and dual $\bbv^*$ arguments.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  L   E   M   M   A   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lemma_important}
%%%
Consider the DSA algorithm as defined in \eqref{eqn_sag_update}-\eqref{initial_DSA_local} and recall the updates of the primal $\bbx^t$ and dual $\bbv^t$ variables in \eqref{DSA_primal_update} and \eqref{DSA_dual_update}, respectively. Further, define the positive semidefinite matrix $\bbU:=(\tbZ-\bbZ)^{1/2}$. If Assumption \ref{ass_wight_matrix_conditions} holds true, then the sequence of primal $\bbx^t$ and dual $\bbv^t$ variables satisfy 
%%%
\begin{align}\label{claim_10}
\alpha \left[\hbg^{t} -\nabla f(\bbx^*)  \right] =(\bbI+\bbZ-2\tbZ)(\bbx^*-\bbx^{t+1})+\tbZ(\bbx^{t}-\bbx^{t+1}) -\bbU(\bbv^{t+1}-\bbv^*).
\end{align}
%%%
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
Considering the update rule for the dual variable in \eqref{DSA_dual_update} and the definition $\bbU=(\tbZ-\bbZ)^{1/2}$, we can substitute $\bbU\bbv^t$ in \eqref{DSA_primal_update} by $\bbU\bbv^{t+1}-\bbU^2\bbx^{t+1}$. Applying this substitution into the DSA primal update in \eqref{DSA_primal_update} yields
%%
%%
\begin{equation}\label{combine_20}
\alpha \hbg^{t}
= -(\bbI+\bbZ-\tbZ)\bbx^{t+1}+\tbZ\bbx^{t}-\bbU\bbv^{t+1}.
\end{equation}
%%
By adding and subtracting $\tbZ\bbx^{t+1}$ into the right hand side of \eqref{combine_20} and considering the fact that $(\bbI+\bbZ-2\tbZ)\bbx^{*}=\bb0$ we obtain 
%%
\begin{equation}\label{combine_30}
\alpha \hbg^{t}
= (\bbI+\bbZ-2\tbZ)(\bbx^*-\bbx^{t+1})+\tbZ(\bbx^{t}-\bbx^{t+1})-\bbU\bbv^{t+1}.
\end{equation}
%%
One of the KKT conditions of problem \eqref{constrained_opt_problem} follows that the optimal variables $\bbx^*$ and $\bbv^*$ satisfy $\alpha\nabla f(\bbx^*)+\bbU\bbv^*=\bb0$ or equivalently $-\alpha \nabla f(\bbx^*)=\bbU\bbv^{*}$. Adding this equality to both sides of \eqref{combine_30} follows the claim in \eqref{claim_10}. 
%
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    M  A   I  N         M   A    T   T   E   R  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the subsequent analyses of convergence of DSA, we need an upper bound for the expected value of squared difference between the stochastic averaging gradient $\hbg^t$ and the gradient of optimal argument $\nabla f(\bbx^*)$ given the observation until step $t$, i.e. $\E{\left\|   \hbg^{t}    -    \nabla f(\bbx^*) \right\|^2  \mid \ccalF^t}$. To establish this upper bound first we define the sequence $p^{t}\in \reals$ as
%%
\begin{align}\label{p_definition}
p^{t}:= \sum_{n=1}^N
\bigg[ 
\frac{1}{q_n}\sum_{i=1}^{q_n}\left( f_{n,i}(\bby_{n,i}^{t}) - f_{n,i}(\tbx^*) -\nabla f_{n,i}(\tbx^*)^T (\bby_{n,i}^{t}-\tbx^*)\right)
 \bigg].
\end{align}
%%
Notice that based on strong convexity of local instantaneous functions $f_{n,i}$, each term $f_{n,i}(\bby_{n,i}^{t}) - f_{n,i}(\tbx^*) 
-\nabla f_{n,i}(\tbx^*)^T (\bby_{n,i}^{t}-\tbx^*)$ is positive and as a result the sequence $p^t$ defined in \eqref{p_definition} is always positive. In the following lemma, we use the result in Lemma \ref{lemma_important} to guarantee an upper bound for the expectation $\E{\|  \hbg^{t} -\nabla f(\bbx^*) \|^2  \mid \ccalF^t}$ in terms of $p^t$ and the optimality gap $f(\bbx^{t}) - f(\bbx^*)  -\nabla f(\bbx^*)^T (\bbx^{t}-\bbx^*)$.










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  L   E   M   M   A   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lemma_gradient_noise_bound}
%%%
%%%
Consider the DSA algorithm in \eqref{eqn_sag_update}-\eqref{initial_DSA_local} and the definition of sequence $p^t$ in \eqref{p_definition}. If Assumptions \ref{ass_wight_matrix_conditions}-\ref{ass_bounded_stochastic_gradient_norm} hold true, then the squared norm of the difference between stochastic averaging gradient  $\hbg^{t}$ and the optimal gradient $\nabla f(\bbx^*)$ in expectation is bounded above by
%%%%
\begin{align}\label{claim_gradient_noise}
\E{\left\|   \hbg^{t}    -    \nabla f(\bbx^*) \right\|^2  
\!\mid\! \ccalF^t}	 \leq 
			4Lp^t
+2\left(2 L -\mu\right)  \left(f(\bbx^{t}) - f(\bbx^*)  -\nabla f(\bbx^*)^T (\bbx^{t}-\bbx^*)\right).
\end{align}
%%
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
See Appendix \ref{apx_lemma_grad_noise_bound}.
\end{proof}


Observe that as the sequence of iterates $\bbx^t$ approaches the optimal argument $\bbx^*$, all the local auxiliary variables $\bby_{n,i}^t$ converge to $\tbx^*$ which follows convergence of $p^t$ to null. This observation in association with the result in \eqref{claim_gradient_noise} implies that the expected value of the difference between the stochastic averaging gradient $\hbg^{t}  $ and the optimal gradient $\nabla f(\bbx^*)$ vanishes as the sequence of iterates $\bbx^t$ approaches the optimal argument $\bbx^*$.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%   S   E    C    T      I     O    N     %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Convergence}

In this section we establish linear convergence of the sequence of iterates $\bbx^t$ generated by DSA to the optimal argument $\bbx^*$. To do so define $0<\gamma $ and $\Gamma<\infty$ as the smallest and largest eigenvalues of positive definite matrix matrix $\tbZ$, respectively. Likewise, define $\gamma'$ as the smallest non-zero eigenvalue of matrix $\tbZ-\bbZ$ and $\Gamma'$ as the largest eigenvalue of matrix $\tbZ-\bbZ$. Further, define vectors $\bbu^{t},\bbu^*\in \reals^{2Np}$ and matrix $\bbG\in \reals^{2Np\times 2Np}$ as
%%
\begin{equation}\label{z_G_definitions}
\bbu^*:=
\begin{bmatrix}
\bbx^*\\ \bbv^*
\end{bmatrix}
, \quad 
\bbu^t:=
\begin{bmatrix}
\bbx^t\\ \bbv^t
\end{bmatrix}
%%
,\quad
%%
\bbG
=
\begin{bmatrix}
    \tbZ & \bb0 \\
    \bb0 & \bbI
\end{bmatrix}.
\end{equation}
%%
Vector $\bbu^*\in \reals^{2Np}$ concatenates the optimal primal and dual variables and vector $\bbu^t\in \reals^{2Np}$ contains primal and dual iterates at step $t$. Matrix $\bbG\in \reals^{2Np\times 2Np}$ is a block diagonal positive definite matrix that we introduce since  instead of tracking the value of $\ell_2$ norm  $\|\bbu^{t}-\bbu^{*}\|^2_{2}$ we study the convergence properties of $\bbG$ weighted norm $\|\bbu^{t}-\bbu^{*}\|^2_{\bbG}$. Notice that the weighted norm $\|\bbu^{t}-\bbu^{*}\|^2_{\bbG}$ is equivalent to $(\bbu^{t}-\bbu^{*})^T\bbG(\bbu^{t}-\bbu^{*})$. Our goal is to show that the sequence $\|\bbu^{t}-\bbu^{*}\|^2_{\bbG}$ converges linearly to null. To do this we show linear convergence of a Lyapunov function of the sequence $\|\bbu^{t}-\bbu^{*}\|^2_{\bbG}$. The Lyapunov function is defined as $\|\bbu^{t}-\bbu^{*}\|^2_{\bbG}+c p^t$ where $c>0$ is a positive constant.






To prove linear convergence of the sequence $\|\bbu^{t}-\bbu^{*}\|^2_{\bbG}+c p^t$ we first show an upper bound for the expected error $\E{\|\bbu^{t+1}-\bbu^{*}\|^2_{\bbG}\mid \ccalF^t}$ in terms of $\|\bbu^{t}-\bbu^{*}\|^2_{\bbG}$ and some parameters that capture the optimality gap.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  L   E   M   M   A   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lemma_lower_bound_for_z_decrement}
%%%
%%%
Consider the DSA algorithm as defined in \eqref{eqn_sag_update}-\eqref{initial_DSA_local}. Further recall the definitions of $p^t$ in \eqref{p_definition} and $\bbu^t$, $\bbu^*$, and $\bbG$ in \eqref{z_G_definitions}. If Assumptions \ref{ass_wight_matrix_conditions}-\ref{ass_bounded_stochastic_gradient_norm} hold true, then for any positive constants $\eta>0$ we can write 
%%%
\begin{align}\label{claim_z_decrement_prime}
	\E{\|\bbu^{t+1}-\bbu^*\|_\bbG^2\mid \ccalF^t}	&\leq
\|\bbu^t-\bbu^*\|_\bbG^2
-2\E{\|\bbx^{t+1}-\bbx^*\|_{\bbI+\bbZ-2\tbZ}^2\mid \ccalF^t}
	+\frac{\alpha4L}{\eta}p^t
\nonumber
\\
&\quad 	-\E{\|\bbx^{t+1}-\bbx^t\|_{\tbZ-2\alpha\eta\bbI}^2\mid \ccalF^t}
	-\E{\|\bbv^{t+1}-\bbv^t\|^2\mid \ccalF^t}\nonumber\\
&   \quad  
	 -\left(\frac{4\alpha\mu }{L} -   \frac{2\alpha( 2L-\mu)}{\eta}  \right)
\left(
 f(\bbx^{t}) - f(\bbx^*)  -\nabla f(\bbx^*)^T (\bbx^{t}-\bbx^*)\right).
\end{align}
%%%.
\end{lemma}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
See Appendix \ref{apx_lemma_lower_bound_for_z_decrement}.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    M  A   I  N         M   A    T   T   E   R  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Lemma \ref{lemma_lower_bound_for_z_decrement} shows an upper bound for the squared norm $\|\bbu^{t+1}-\bbu^{*}\|^2_{\bbG}$ which is the first part of the Lyapunov function $\|\bbu^{t}-\bbu^{*}\|^2_{\bbG}+c p^t$ at step $t+1$. Likewise, we provide an upper bound for the second term of the Lyapunov function at time $t+1$ which is $p^{t+1}$ in terms of $p^{t}$ and some parameters that capture optimality gap. This bound is studied in the following lemma.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  L   E   M   M   A   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lemma_p_decrement_2}
%%
Consider the DSA algorithm as defined in \eqref{eqn_sag_update}-\eqref{initial_DSA_local} and the definition of $p^t$ in \eqref{p_definition}. Further, define $q_{\min}$ and $q_{\max}$ as the smallest and largest values for the number of instantaneous functions at a node, respectively. If Assumptions \ref{ass_wight_matrix_conditions}-\ref{ass_bounded_stochastic_gradient_norm} hold true, then for all $t>0$ the sequence $p^t$ satisfies
%%
\begin{align}\label{lemma_p_decrement_claim}
\E{
p^{t+1}
 \mid \ccalF^t}
 \leq
 \left[1-\frac{1}{q_{\max}}\right]p^t+\frac{1}{q_{\min}}\left[ f(\bbx^t)-f(\bbx^*) -\nabla f(\bbx^*)^T (\bbx^{t}-\bbx^*) \right].
\end{align}
%%%
\end{lemma}
%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
See Appendix \ref{apx_lemma_p_decrement_2}.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    M  A   I  N         M   A    T   T   E   R  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Lemma \ref{lemma_p_decrement_2} provides an upper bound for $p^{t+1}$ in terms of its previous value $p^{t}$ and the optimality error $f(\bbx^t)-f(\bbx^*) -\nabla f(\bbx^*)^T (\bbx^{t}-\bbx^*) $. Combining the results in Lemmata \ref{lemma_lower_bound_for_z_decrement} and \ref{lemma_p_decrement_2} we can show that in expectation the Lyapunov function $\| \bbu^{t+1}-\bbu^*\|_\bbG^2+c\ p^{t+1}$ at step $t+1$ is strictly smaller than its previous value  $\| \bbu^{t}-\bbu^*\|_\bbG^2+c\ p^t$ at step $t$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   T   H   E   O   R   E   M   %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{lin_convg_thm}
Consider the DSA algorithm as defined in \eqref{eqn_sag_update}-\eqref{initial_DSA_local}. Further recall the definition of the sequence $p^t$ in \eqref{p_definition}. Define $\eta$ as an arbitrary positive constant chosen from the interval 
%%%
\begin{equation}\label{eta_condition}
\eta\in\left(
 \frac{L^2q_{\max}}{\mu q_{\min} }+\frac{L^2}{\mu}-L\ , \ \infty
\right).
\end{equation}
%%
%%
If Assumptions \ref{ass_wight_matrix_conditions}-\ref{ass_bounded_stochastic_gradient_norm} hold true and the stepsize $\alpha$ is chosen from the interval $\alpha \in \left( 0,  {\gamma}/{2\eta}\right)$,
%%%
%\begin{equation}
% \alpha \in \left( 0\ , \ \frac{\gamma}{2\eta}\right),
%\end{equation}
then for arbitrary $c$ chosen from the interval
%%
\begin{equation}\label{c_condition}
c\in \left( \frac{4\alpha L q_{\max}}{\eta}\ , \ \frac{4\alpha \mu q_{\min}}{L}-\frac{2\alpha q_{\min}(2L-\mu)}{\eta}
\right),
\end{equation}
%%
there exits a positive constant $0<\delta<1$ such that 
%%
\begin{equation}\label{linear_convg_claim}
\E{\|\bbu^{t+1}-\bbu^{*}\|^2_{\bbG}+c\ \! p^{t+1} \mid \ccalF^t}\leq  (1-\delta)\left(\|\bbu^{t}-\bbu^{*}\|^2_{\bbG}+c\ \! p^t\right).
\end{equation}
%%
\end{theorem}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
See Appendix \ref{apx_lin_convg_thm}.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    M  A   I  N         M   A    T   T   E   R  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We point out that the linear convergence constant $\delta$ in \eqref{linear_convg_claim} is explicitly available -- see \eqref{linear_convg_70} in Appendix \ref{apx_lin_convg_thm}. It is a function of the strong convexity parameter $\mu$, the Lipschitz continuity constant $L$, lower and upper bounds on the eigenvalues of the matrices $\tbZ$, $\tbZ-\bbZ$, and $\bbI+\bbZ-2\tbZ$, the smallest $q_{\min}$ and largest $q_{\max}$ values for the number of instantaneous functions available at a node, and the stepsize $\alpha$. Insight on the dependence of $\delta$ with problem parameters is offered in Section \ref{sec_convergence_constant}.

The inequality in \eqref{linear_convg_claim} shows that the expected value of the sequence $\|\bbu^{t}-\bbu^{*}\|^2_{\bbG}+c\ \! p^t$ at time $t+1$ given the observation until step $t$ is strictly smaller than the previous iterate at step $t$. Computing the expected value with respect to the initial sigma field $\E{.\mid \ccalF^0}=\E{.}$ implies that in expectation the sequence $\|\bbu^{t}-\bbu^{*}\|^2_{\bbG}+c\ \! p^t$ converges linearly to null, i.e.,
%%
\begin{equation}\label{best_result}
\E{\|\bbu^{t}-\bbu^{*}\|^2_{\bbG}+c\ \! p^{t}}\leq  (1-\delta)^{t} \left(\|\bbu^{0}-\bbu^{*}\|^2_{\bbG}+c\ \! p^0\right).
\end{equation}
%%
We use the result in \eqref{best_result} to establish linear convergence of the sequence of squared norm error $\|\bbx^t-\bbx^*\|^2$ in expectation. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%      C   O    R    O    L    L     A     R   Y     %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{corollary}\label{corollary_lin_convg}
Consider the DSA algorithm as defined in \eqref{eqn_sag_update}-\eqref{initial_DSA_local} and recall $\gamma$ is the minimum eigenvalue of the positive definite matrix $\tbZ$. If the hypothesis of Theorem \ref{lin_convg_thm} holds, then there exits a positive constant $0<\delta<1$ such that 
\begin{equation}\label{best222}
\E{\|\bbx^{t}-\bbx^{*}\|^2}\leq  (1-\delta)^{t} \frac{\left(\|\bbu^{0}-\bbu^{*}\|^2_{\bbG}+c\ \! p^0\right).}{\gamma}
\end{equation}
\end{corollary}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
First note that according to the definitions of $\bbu$ and $\bbG$ in \eqref{z_G_definitions} and the definition of $p^t$ in \eqref{p_definition} , we can write $\|\bbx^{t}-\bbx^{*}\|_{\tbZ}^2\leq \|\bbu^{t}-\bbu^{*}\|^2_{\bbG}+c\ \! p^{t}$. Further, note that the weighted norm $\|\bbx^{t}-\bbx^{*}\|_{\tbZ}^2$ is lower bounded by $\gamma\|\bbx^{t}-\bbx^{*}\|^2$, since $\gamma$ is a lower bound for the eigenvalues of $\tbZ$. Combine these two observations to obtain $\gamma\|\bbx^{t}-\bbx^{*}\|^2\leq \|\bbu^{t}-\bbu^{*}\|^2_{\bbG}+c\ \! p^{t}$. This inequality in conjunction with the expression in \eqref{best_result} follows the claim in \eqref{best222}.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    M  A   I  N         M   A    T   T   E   R  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Corollary \ref{corollary_lin_convg} states that the sequence $\E{\|\bbx^{t}-\bbx^{*}\|^2}$ linearly converges to null. Note that the sequence $\E{\|\bbx^{t}-\bbx^{*}\|^2}$ is not necessarily monotonically decreasing as the sequence $\E{\|\bbu^{t}-\bbu^{*}\|^2_{\bbG}+c\ \! p^t}$ is. The result in \eqref{best222} shows linear convergence of the sequence of variables generated by DSA in expectation. In the following Theorem we show that all local variables $\bbx_n^t$ generated by DSA almost surely converge to the optimal argument of \eqref{opt_problem}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   T   H   E   O   R   E   M   %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{a_s_convg}
Consider the DSA algorithm as defined in \eqref{eqn_sag_update}-\eqref{initial_DSA_local} and assume the same hypothesis of Theorem \ref{lin_convg_thm}.
Then, the sequences of local variables $\bbx_{n}^t$ for all $n=1,\dots, N$ converge almost surely to the optimal argument $\tbx^*$, i.e., 
%%
\begin{equation}\label{a_s_convg_claim}
\lim_{t \to \infty} \bbx_n^t\ = \ \tbx^* \quad a.s.  \qquad \forall\  n=1,\dots, N.
\end{equation}
%%
Further, the almost sure convergence is at least of order $\ccalO(1/t)$.
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
See Appendix \ref{apx_a_s_convg}.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    M  A   I  N         M   A    T   T   E   R  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Theorem \ref{a_s_convg} provides almost sure convergence of $\bbx^t$ to the optimal solution $\bbx^*$ which is stronger result than convergence in expectation as in Corollary \ref{corollary_lin_convg}, however, the rate of convergence for the almost sure convergence is  sublinear $\ccalO(1/t)$ which is slower relative to the linear convergence in expectation provided in \eqref{best222}.




\subsection{Convergence constant}\label{sec_convergence_constant}

The constant $\delta$ that controls the speed of convergence can be simplified by selecting specific values for $\eta$, $\alpha$, and $c$. This uncovers connections to the properties of the local objective functions and the network topology. To make this clearer define the condition numbers of the objective function and the graph as 
 %%
 \begin{equation}\label{condition_numbers}
 \kappa_f=\frac{L}{\mu}, \qquad \kappa_g=\frac{\max\{\Gamma,\Gamma'\}}{\min\{\gamma,\gamma'\}},
 \end{equation} 
%%
respectively. The condition number of the function is a measure of how difficult it is to minimize the local functions using gradient descent directions. The condition number of the graph is a measure of how slow the graph is in propagating a diffusion process. Both are known to control the speed of convergence of distributed optimization methods. The following corollary illustrates that these condition numbers also determine the convergence speed of DSA.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%      C   O    R    O    L    L     A     R   Y     %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{corollary}\label{corollary_lin_convg_constant}
Consider the DSA algorithm as defined in \eqref{eqn_sag_update}-\eqref{initial_DSA_local} and assume the same hypothesis of Theorem \ref{lin_convg_thm}. Choose the weight matrices $\bbW$ and $\tbW$ as $\tbW=(\bbI+\bbW)/2$, assign the same number of instantaneous local functions $f_{n,i}$ to each node, i.e., $q_{\min}=q_{\max}=q$, and set the constants $\eta$, $\alpha$ and $c$ as
%%%
\begin{equation}\label{constants}
\eta=\frac{2L^2}{\mu}, \quad \alpha=\frac{\gamma\mu}{8L^2},\quad 
c=\frac{q\gamma \mu^2}{4L^3}\left( 1+\frac{\mu}{4L} \right).
\end{equation}
%%%
The linear convergence constant $0<\delta<1$ in \eqref{linear_convg_claim} reduces to
%%%%
\begin{equation}\label{something}
\delta = \min \Bigg[\frac{1}{ 16\kappa_g^2}, \
\frac{1}{q[1+4\kappa_f(1+\gamma/\gamma')]},\
\frac{1}{ 4(\gamma/\gamma')\kappa_f+32\kappa_g\kappa_f^4 }
\Bigg].
\end{equation}
%%
\end{corollary}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
The given values for $\eta$, $\alpha$, and $c$ satisfy the conditions in Theorem \ref{lin_convg_thm}. Substitute then these values into the expression for $\delta$ in \eqref{linear_convg_70}. Simplify terms and utilize the condition number definitions in \eqref{condition_numbers}. The second term in the minimization in \eqref{linear_convg_70} becomes redundant because it is dominated by the first.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%    M  A   I  N         M   A    T   T   E   R  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Observe that while the choices of $\eta$, $\alpha$, and $c$ in \eqref{constants} satisfy all the required conditions of Theorem \ref{lin_convg_thm}, they are not necessarily optimal for maximizing the linear convergence constant $\delta$. Nevertheless, the expression in \eqref{something} shows that the convergence speed of DSA decreases with increases in the graph condition number $\kappa_g$, the local functions condition number $\kappa_f$, and the number of functions assigned to each node $q$. For a cleaner expression observe that both, $\gamma$ and $\gamma'$ are the minimum eigenvalues of the weight matrix $\bbW$ and the weight matrix difference $\tbW-\bbW$. They can therefore be chosen to be of similar order. For reference, say that we choose $\gamma=\gamma'$ so that the ratio $\gamma/\gamma'=1$. In that case, the constant $\delta$ in \eqref{something} reduces to
%%
\begin{equation}\label{approx_constant}
\delta = \min \Bigg[
\frac{1}{16 \kappa_g^2},\
\frac{1}{q(1+8\kappa_f)},\
\frac{1}{4(\kappa_f+8\kappa_f^4\kappa_g)}
\Bigg].
\end{equation}
%%
The three terms in \eqref{approx_constant} establish separate regimes, problems where the graph condition number is large, problems where the number of functions at each node is large, and problems where the condition number of the local functions are large. In the first regime the first term in \eqref{approx_constant} dominates and establishes a dependence in terms of the square of the graph's condition number. In the second regime the middle term dominates and results in an inverse dependence with the number of functions available at each node. In the third regime, the third term dominates. The dependence in this case is inversely proportional to $\kappa_f^4$.









































==> Problem-1.tex <==
%!TEX root = root.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Decentralized Double stochastic averaging gradient }\label{sec:DSA}

Consider a connected network that contains $N$ nodes such that each node $n$ can only communicate with peers in its neighborhood $\ccalN_{n}$. Define $\bbx_n\in \reals^p$ as a local copy of the variable $\bbx$ that is kept at node $n$. In decentralized optimization, agents try to minimize their local functions $f_{n}(\bbx_n)$ while ensuring that their local variables $\bbx_n$ coincide with the variables $\bbx_{m}$ of all neighbors $m \in \ccalN_{n}$ -- which, given that the network is connected, ensures that the variables $\bbx_n$ of all nodes are the same and renders the problem equivalent to \eqref{opt_problem}. DGD is a well known method for decentralized optimization that relies on the introduction of nonnegative weights $w_{ij}\geq0$ that are not null if and only if  $m=n$ or if $m\in \mathcal{N}_n$. Letting $t\in\naturals$ be a discrete time index and $\alpha$ a given stepsize, DGD is defined by the recursion
%
\begin{equation}\label{gd_iteration}
   \bbx_{n}^{t+1} 
      = \sum_{m=1}^{N} w_{nm}\bbx_{m}^{t}-\alpha\nabla f_n({\bbx_{n}^{t}}), 
      \qquad n=1,\ldots,N.
\end{equation}
%
Since $w_{nm}=0$ when $m\neq n$ and $m\notin \mathcal{N}_n$, it follows from \eqref{gd_iteration} that node $n$ updates $\bbx_n$ by performing an average over the variables $\bbx_{m}^t$ of its neighbors $m\in \mathcal{N}_n$ and its own $\bbx_{n}^t$, followed by descent through the negative local gradient $-\nabla f_n(\bbx_{n}^t)$. If a constant stepsize is used, DGD iterates $\bbx_{n}^t$ approach a neighborhood of the optimal argument $\tbx^*$ of \eqref{opt_problem} but don't converge exactly. To achieve exact convergence diminishing stepsizes are used but the resulting convergence rate is sublinear (\cite{Nedic2009}). 

EXTRA is a method that resolves either of these issues by mixing two consecutive DGD iterations with different weight matrices and opposite signs. To be precise, introduce a second set of weights $\tdw_{nm}$ with the same properties as the weights $w_{nm}$ and define EXTRA through the recursion
%
\begin{align}\label{local_extra}
    \bbx_n^{t+1} = \bbx_n^{t}
                    + \sum_{m=1}^N w_{nm} \bbx_{m}^t 
                     - \sum_{m=1}^N \tdw_{nm}\bbx_{m}^{t-1}  - \alpha\left [ \nabla f_n(\bbx_n^{t}) 
                                    -\nabla f_n(\bbx_n^{t-1}) \right] , 
                     \quad  n=1,\ldots,N.
\end{align}
%
Observe that \eqref{local_extra} is well defined for $t>0$. For $t=0$ we utilize the regular DGD iteration in \eqref{gd_iteration}. In the nomenclature of this paper we say that EXTRA performs a decentralized double gradient descent step because it operates in a decentralized manner while utilizing a difference of two gradients as descent direction. Minor modification as it is, the use of this gradient difference in lieu of simple gradients, endows EXTRA with exact linear convergence to the optimal argument $\tbx^*$ under mild assumptions (\cite{Shi2014}).

If we recall the definitions of the local functions $f_{n}(\bbx_n)$ and the instantaneous local functions $f_{n,i}(\bbx_n)$ available at node $n$, the implementation of EXTRA requires that each node $n$ computes the {full} gradient of its local objective function $f_n$ at $\bbx_n^t$ as
%
\begin{equation}\label{gradient}
    \nabla f_{n}(\bbx_n^t) 
        = \frac{1}{q_n} \sum_{{i=1}}^{q_n}
               \nabla f_{n,{i}}(\bbx_n^t).
\end{equation}
%
This is computationally expensive when the number of instantaneous functions $q_n$ is large. To resolve this issue, local stochastic gradients can be substituted for the local objective functions gradients in \eqref{local_extra}. These stochastic gradients approximate the gradient $\nabla f_{n}(\bbx_n)$ of node $n$ by randomly choosing one of the instantaneous functions gradients $\nabla f_{n,i}(\bbx_n)$. If we let $i_n^t\in\{1,\ldots q_n\}$ denote a function index that we choose at time $t$ at node $n$ uniformly at random and independently of the history of the process, then the stochastic gradient is defined as 
%
\begin{equation}\label{sto_gradient}
    \hbs_n(\bbx_n^t):= \nabla f_{n,i_n^{t}}(\bbx_n^t).
\end{equation}
%
We can then write a stochastic version of EXTRA by replacing $\nabla f_n(\bbx_n^{t})$ by $\hbs_n(\bbx_n^t)$ and $\nabla f_n(\bbx_n^{t-1})$ by $\hbs_n(\bbx_n^{t-1})$. Such algorithm would have a small computational cost per iteration and, presumably, converge to the optimal argument $\tbx^*$. Here however, we want to design an algorithm with linear convergence rate, and stochastic descent algorithms achieve sublinear rates because of the difference between the stochastic and deterministic descent directions. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure} \centering
\ifcompiletikz \input{figures/average_gradient_update.tex} 
\else \includegraphics[width=\linewidth]{figures/average_gradient_update.pdf}\fi 
\caption{Stochastic averaging gradient table at node $n$. At each iteration $t$ a random local instantaneous gradient $\nabla f_{n,i_n^{t}}(\bby_{n,i_{n}^t}^{t})$ is updated by $\nabla f_{n,i_n^{t}}(\bbx_n^{t})$. The rest of the local instantaneous gradients remain unchanged, i.e., $\nabla f_{n,i}(\bby_{n,i}^{t+1})=\nabla f_{n,i}(\bby_{n,i}^{t})$ for $i\neq i_n^t$. This list is used to compute the stochastic averaging gradient in \eqref{local_stochastic_gradient}.}
\label{fig_sag} \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
To reduce this noise we propose the use of stochastic averaging gradients instead (\cite{defazio2014saga}). The idea is to maintain a list of gradients of all instantaneous functions in which one randomly chosen element is replaced at each iteration and to use an average of the elements of this list for gradient approximation; see Figure \ref{fig_sag}. Formally, define the variable $\bby_{n,i}\in\reals^{p}$ to represent the iterate value the last time that the instantaneous gradient of function $f_{n,i}$ was evaluated. If we let $i_n^t\in\{1,\ldots, q_n\}$ denote the function index chosen at time $t$ at node $n$, as we did in \eqref{sto_gradient}, the variables $\bby_{n,i}$ are updated recursively as 
%
\begin{equation}\label{eqn_sag_update}
  \bby_{n,i}^{t+1} = \bbx_{n}^t,     \quad \text{if\ } i =    i_{n}^t, \qquad
  \bby_{n,i}^{t+1} = \bby_{n,i}^{t}, \quad \text{if\ } i \neq i_{n}^t.
\end{equation}
%
With these definitions in hand we can define the stochastic averaging gradient at node $n$ as
%
\begin{align}\label{local_stochastic_gradient}
   \hbg_{n}^t :=  \nabla f_{n,i_n^{t}}(\bbx_n^t)
                 -\nabla f_{n,i_n^{t}}(\bby_{n,i_{n}^t}^{t})
                 +\frac{1}{q_n}\sum_{i=1}^{q_n}
                  \nabla f_{n,i}(\bby_{n,i}^{t}).
\end{align}
%
Observe that to implement \eqref{local_stochastic_gradient} the gradients $\nabla f_{n,i}(\bby_{n,i}^{t})$ are stored in the local gradient table shown in Figure \ref{fig_sag}. 


The DSA algorithm is a variation of EXTRA that substitutes the local gradients $\nabla f_n(\bbx_n^t)$ in \eqref{local_extra} for the local stochastic average gradients $\hbg_{n}^t$ in \eqref{local_stochastic_gradient},
%
\begin{equation}\label{DSA_local}
   \bbx_n^{t+1} =  \bbx_n^{t} 
                  +\sum_{m=1}^N w_{nm} \bbx_{m}^t 
                  -\sum_{m=1}^N \tdw_{nm} \bbx_{m}^{t-1}
                  - \alpha\left[\hbg_{n}^t-\hbg_{n}^{t-1}\right].
\end{equation}
%
The DSA initial update is given by applying the same substitution for the update of DGD in \eqref{gd_iteration} as
%
\begin{equation}\label{initial_DSA_local}
    \bbx_n^{1}=\sum_{m=1}^N w_{nm} \bbx_{m}^0 - \alpha\ \hbg_{n}^0.
\end{equation}
%
DSA is summarized in Algorithm \ref{algo_DSA} for $t\geq1$. The DSA update in \eqref{DSA_local} is implemented in Step 9. This step requires access to the local iterates $\bbx_m^t$ of  neighboring nodes $m\in \ccalN_{n}$ which are collected in Step 2. Furthermore, implementation of the DSA update also requires access to the stochastic averaging gradients $\hbg_n^{t-1}$ and $\hbg_n^t$. The latter is computed in Step 4 and the former is computed and stored at the same step in the previous iteration. The computation of the stochastic averaging gradients requires the selection of the index $i_{n}^t$. This index is chosen uniformly at random in Step 3. Determination of stochastic averaging gradients also necessitates access and maintenance of the gradients table in Figure \ref{fig_sag}. The $i_n^t$ element of this table is updated in Step 5 by replacing $\nabla f_{n,i_n^t}(\bby_{n,i_{n}^t}^t)$ with $\nabla f_{n,i_n^t}(\bbx_n^t)$, while the other vectors remain unchanged. To implement the first DSA iteration at time $t=0$ we have to perform the update in \eqref{initial_DSA_local} instead of the update in \eqref{DSA_local} as in Step 7. Furhter observe that the auxiliary variables $\bby_{n,i}^0$ are initialized to the initial iterate $\bbx_n^0$. This implies that the initial values of the stored gradients are $\nabla f_{n,i}(\bby_{n,i}^0) = \nabla f_{n,i}(\bbx_n^0)$ -- with a consequently relatively large initialization cost.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%   A   L   G   O   R   I   T   H   M   %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%\begin{algorithm}[tb]
%\caption{DSA algorithm at node $n$}\label{algo_DSA} 
%\begin{algorithmic}[1] 
%\small{\REQUIRE Vectors $\bbx_{n}^0$, $\bbx_{n}^1$, and $\hbg_{n}^{0}$. Gradient table initialized with instantaneous gradients $\nabla f_{n,i}(\bby_{n,i}^1)$ with $\bby_{n,i}^0 = \bbx_n^0$. 
%%
%\FOR {$t=1,2,\ldots$}
%   \STATE Exchange variable $\bbx_{n}^t$ with neighboring nodes $m\in \ccalN_n$.
%   \STATE Choose $i_{n}^t$ uniformly at random from the set $\{1,\dots,q_{n}\}$.
%   \STATE Compute and store stochastic averaging gradient as per \eqref{local_stochastic_gradient}\\
%          $ \displaystyle{\hbg_{n}^t
%                 =  \nabla f_{n,i_n^{t}}(\bbx_{n}^t)
%                  -\nabla f_{n,i_n^{t}}(\bby_{n,i_{n}^t}^{t}) 
%                  +\frac{1}{q_n} \sum_{i=1}^{q_n} 
%                   \nabla f_{n,i}(\bby_{n,i}^{t}) }$
%   \STATE Store $\nabla f_{n,i_{n}^t}(\bby_{n,i_{n}^t}^{t+1}) 
%          = \nabla f_{n,i_{n}^t}(\bbx_{n}^t)$ in $i_{n}^t$ 
%          gradient table position
%   \STATE Update variable $\bbx_{n}^t$ as per \eqref{DSA_local}\\       %
%%  \IF{$t=0$}
%%     \STATE    
%%     $\displaystyle{\bbx_n^{t+1}=\sum_{n=1}^{N}w_{nm}\bbx_n^{t+1}- \alpha \hbg_{n}^t.}$
%%  \ELSE
%%     \STATE    
%          $\displaystyle{\bbx_n^{t+1} 
%              = \bbx_n^{t} + \sum_{n=1}^{N}w_{nm}\bbx_n^{t} 
%                           - \sum_{n=1}^{N}\tilde{w}_{nm}\bbx_n^{t-1}
%                           - \alpha\left[\hbg_{n}^t-\hbg_{n}^{t-1}\right].}$
%%  \ENDIF
%\ENDFOR}
%\end{algorithmic}\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   L   G   O   R   I   T   H   M   %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{algorithm}[tb]
\caption{DSA algorithm at node $n$}\label{algo_DSA} 
\begin{algorithmic}[1] 
\small{\REQUIRE Vectors $\bbx_{n}^0$. Gradient table initialized with instantaneous gradients $\nabla f_{n,i}(\bby_{n,i}^0)$ with $\bby_{n,i}^0 = \bbx_n^0$. 
%
\FOR {$t=0,1,2,\ldots$}
   \STATE Exchange variable $\bbx_{n}^t$ with neighboring nodes $m\in \ccalN_n$.
   \STATE Choose $i_{n}^t$ uniformly at random from the set $\{1,\dots,q_{n}\}$.
   \STATE Compute and store stochastic averaging gradient as per \eqref{local_stochastic_gradient}:\\
          $ \displaystyle{\hbg_{n}^t
                 =  \nabla f_{n,i_n^{t}}(\bbx_{n}^t)
                  -\nabla f_{n,i_n^{t}}(\bby_{n,i_{n}^t}^{t}) 
                  +\frac{1}{q_n} \sum_{i=1}^{q_n} 
                   \nabla f_{n,i}(\bby_{n,i}^{t}) .}$
   \STATE Store $\nabla f_{n,i_{n}^t}(\bby_{n,i_{n}^t}^{t+1}) 
          = \nabla f_{n,i_{n}^t}(\bbx_{n}^t)$ in $i_{n}^t$ .
          gradient table position. %
  \IF{$t=0$}
  \vspace{-1.5mm}
     \STATE     Update variable $\bbx_{n}^t$ as per \eqref{initial_DSA_local}: 
     $\quad \displaystyle{\bbx_n^{t+1}=\sum_{n=1}^{N}w_{nm}\bbx_n^{t+1}- \alpha \hbg_{n}^t.}$
       \vspace{-1.5mm}
  \ELSE
    \vspace{-1.5mm}
     \STATE    Update variable $\bbx_{n}^t$ as per \eqref{DSA_local}:
          $\quad \displaystyle{\bbx_n^{t+1} 
              = \bbx_n^{t} + \sum_{n=1}^{N}w_{nm}\bbx_n^{t} 
                           - \sum_{n=1}^{N}\tilde{w}_{nm}\bbx_n^{t-1}
                           - \alpha\left[\hbg_{n}^t-\hbg_{n}^{t-1}\right].}$
                             \vspace{-1.5mm}
  \ENDIF
\ENDFOR}
\end{algorithmic}\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

We point out that the weights $w_{nm}$ and $\tdw_{nm}$ can't be arbitrary. If we define  weight matrices $\bbW$ and $\tbW$ with elements $w_{nm}$ and $\tdw_{nm}$, respectively, they have to satisfy conditions that we state as an assumption for future reference.
\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   S   S   U   M   P   T   I   O   N   %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{assumption}\label{ass_wight_matrix_conditions}
The weight matrices $\bbW$ and $\tbW$ must satisfy the following properties
\begin{mylist}
\item[(a)] Both are symmetric, $\bbW=\bbW^T$ and $\tbW=\tbW^T$. \label{symmetry}
%
\item[(b)] The null space of $\bbI-\tbW$ includes the span of $\bbone$, i.e., $\text{null}(\bbI-\tbW)\supseteq \text{span}(\bbone)$, the null space of $\bbI-\bbW$ is the span of $\bbone$, i.e., $\text{null}(\bbI-\tbW)= \text{span}(\bbone)$, and the null space of the difference $\tbW-\bbW$ is the span of $\bbone$, i.e., $\text{null}(\tbW-\bbW)=\text{span}(\bbone)$. \label{spectral1}
%
\item[(c)] They satisfy the spectral ordering $ \bbW \preceq  \tbW \preceq ({\bbI+\bbW})/{2}$ and the matrix $\tbW$ is positive definite $\bb0\prec\tbW$.  \label{spectral2}
\end{mylist} \end{assumption}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M  A   I  N         M   A    T   T   E   R  %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Requiring the matrix $\bbW$ to be symmetric and with specific null space properties is necessary to let all agents converge to the same optimal variable. Analogous properties are necessary in DGD and are not difficult to satisfy. The condition on spectral ordering is specific to EXTRA but is not difficult to satisfy either. {E.g., if we have a matrix $\bbW$ that satisfies all the conditions in Assumption \ref{ass_wight_matrix_conditions}, the weight matrix $\tbW=(\bbI+\bbW)/2$ makes Assumption \ref{ass_wight_matrix_conditions} valid.} %\blue{Watch out, not exactly true. You need $\text{null}(\bbI-\tbW)\supseteq \text{span}(\bbone)$ to have $\text{null}(\tbW-\bbW)=\text{span}(\bbone)$. With this choice of $\tbW$ the null spaces are the same. Change the assumption?} \red{Conditions on the spectral properties of matrices $\bbW$ and $\tbW$ in Assumptions \ref{ass_wight_matrix_conditions}\eqref{spectral1} and \ref{ass_wight_matrix_conditions}\eqref{spectral2} imply that the null space of matrix $\bbI-\bbW$ is span of vector $\bold{1}$, i.e. null$\{\bbI-\bbW\}=$ span$\{\bold{1}\}$ -- see Proposition 2.1 \cite{Shi2014}.} \blue{This is not important. Mention it in the proofs, where you use the result.}

We also point that, as written in \eqref{local_stochastic_gradient}, computation of local stochastic averaging gradients $\hbg_n^t$ is costly because it requires evaluation of the sum $\sum_{i=1}^{q_n}\nabla f_{n,i}(\bby_{n,i}^{t})$ at each iteration. This cost can be avoided by updating the sum at each iteration with the recursive formula 
%
\begin{align}\label{local_stochastic_gradient_recursive}
 \sum_{i=1}^{q_n}\nabla f_{n,i}(\bby_{n,i}^{t}) 
 	   \ =\  \sum_{i=1}^{q_n}\nabla f_{n,i}(\bby_{n,i}^{t-1}) 
           + \nabla f_{n,i_n^{t-1}}(\bbx_n^{t-1})
                        -\nabla f_{n,i_n^{t-1}}(\bby_{n,i_{n}^{t-1}}^{t-1}) .
\end{align}
%
Important properties and interpretations of EXTRA and DSA are presented in the following sections after a pertinent remark.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   R   E   M    A     R   K   %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{remark}\label{rmk_unbiased_estimation}\normalfont The local stochastic averaging gradients in \eqref{local_stochastic_gradient} are unbiased estimates of the local gradients $\nabla f_{n}(\bbx_n^t)$. Indeed, if we let $\ccalF_t$ measure the history of the system up until time $t$ we have that the sum in \eqref{local_stochastic_gradient} is deterministic given this sigma-algebra. Thus, the conditional expectation of the stochastic averaging gradient is, 
%
\begin{align}\label{expected_value_simplification_intermediate}
   \E{\hbg_{n}^t\given\ccalF^t} 
       = \mbE\Big[\nabla f_{n,i_n^{t}}(\bbx_n^t)\given\ccalF^t\Big]
                 -\mbE\Big[\nabla f_{n,i_n^{t}}(\bby_{n,i_{n}^t}^{t})\given\ccalF^t\Big]
                 +\frac{1}{q_n}\sum_{i=1}^{q_n}
                  \nabla f_{n,i}(\bby_{n,i}^{t}).
\end{align}
%
With the index $i_n^t$ chosen equiprobably from the set $\{1,\ldots, q_n\}$, the expectation of the second term in \eqref{expected_value_simplification_intermediate} is the same as the sum in the last term -- each of the indexes is chosen with probability $1/q_n$. Therefore, these two terms cancel out each other and, since the expectation of the first term in \eqref{expected_value_simplification_intermediate} is simply $\mbE\big[\nabla f_{n,i_n^{t}}(\bbx_n^t)\given\ccalF^t\big] = (1/q_n) \sum_{i=1}^{q_n}\nabla f_{n,i}(\bbx_n^t) =\nabla f_{n}(\bbx_n^t)$, we can simplify \eqref{expected_value_simplification_intermediate} to
%
\begin{align}\label{expected_value_simplification}
   \E{\hbg_{n}^t\given\ccalF^t} = \nabla f_{n}(\bbx_n^t).
\end{align}
%
The expression in \eqref{expected_value_simplification} means, by definition, that $\hbg_{n}^t$ is an unbiased estimate of $\nabla f_{n}(\bbx_n^t)$ when the history $\ccalF^t$ is given.
\end{remark}











==> Rate.tex <==
%!TEX root = root.tex
%\subsection{Rate of Convergence} \label{sec:rate}\vspace{-2mm}
%\red{In this section we investigate the rate of convergence for the regularized stochastic BFGS. In \cite{Dennis,Powell,Byrd, Nocedal} it has been shown that the rate of convergence for deterministic BFGS is super-linear under the condition that the sequence of step sizes is chosen based on some line search algorithms, e.g. Wolfe conditions. In stochastic settings line searches are problematic, since the value of descent function is not available for all the points. As a consequence in stochastic optimization constant or diminishing step sizes are applied which avoids achieving a super-linear rate of convergence. In the following Theorem we show that the rate of convergence for regularized stochastic BFGS in terms of expectation of the objective function error is linear.} \blue{This is just a long excuse for not proving a stronger result. Just say what the theorem claims and that's it.}
We complement the convergence result in Theorem \ref{convg} with a characterization of the expected convergence rate that we introduce in the following theorem.
%
\begin{theorem}\label{theo_convergence_rate}
Consider the online Limited memory BFGS algorithm as defined by \eqref{eqn_olbfgs_descent}-\eqref{initial_matrix_update_2}. If assumptions \ref{ass_intantaneous_hessian_bounds}, \ref{ass_bounded_stochastic_gradient_norm} and \ref{stepsize_ass} hold true and the step size parameters $\eps_0$ and $T_{0}$ satisfy the inequality
%
\begin{equation}\label{eqn_thm_cvg_rate_10}
    2\  \epsilon_{0} T_{0} \delta >1\ ,
\end{equation} 
%
then the optimal objective $F(\bbw^*)$ satisfies 
%
\vspace{-2mm}
\begin{equation}\label{eqn_thm_cvg_rate_20}
\E {F(\bbw_{t})}- F(\bbw^*)\ \leq\ \frac{C_{0}}{T_{0}+t}\ ,\vspace{-2mm}
\end{equation}
%
where the constant $C_{0}$ satisfies
%
\vspace{-2mm}
\begin{equation}\label{eqn_thm_cvg_rate_30}
 C_{0} = \max \left\{ \frac{\epsilon_{0}^{2}\   T_{0}^{2} K}{2 \epsilon_{0} T_{0} \delta -1}, T_{0}\ \!  (F(\bbw_{0}) -\ F(\bbw^*))  \right\} .\vspace{-2mm}
\end{equation}
%
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Proof of Theorem 2
%
%\begin{proof} 
%See Supplementary Material.
 %\end{proof}

Theorem \ref{theo_convergence_rate} shows that under specified assumptions, the expected error  in terms of the objective value after $t$ oLBFGS iterations is of order $O(1/t)$. This implies that the rate of convergence for oLBFGS is not better than conventional SGD. While the convergence rate doesn't change, improvements in convergence time are marked as we illustrate with the numerical experiments of section \ref{sec_ad_numerical_results}.



